In-Context Ability Transfer for Question Decomposition in Complex QA

Answering complex questions is a challenging task that requires question decomposition and multistep reasoning for arriving at the solution. While existing supervised and unsupervised approaches are specialized to a certain task and involve training, recently proposed prompt-based approaches offer generalizable solutions to tackle a wide variety of complex question-answering (QA) tasks. However, existing prompt-based approaches that are effective for complex QA tasks involve expensive hand annotations from experts in the form of rationales and are not generalizable to newer complex QA scenarios and tasks. We propose, icat (In-Context Ability Transfer) which induces reasoning capabilities in LLMs without any LLM fine-tuning or manual annotation of in-context samples. We transfer the ability to decompose complex questions to simpler questions or generate step-by-step rationales to LLMs, by careful selection from available data sources of related tasks. We also propose an automated uncertainty-aware exemplar selection approach for selecting examples from transfer data sources. Finally, we conduct large-scale experiments on a variety of complex QA tasks involving numerical reasoning, compositional complex QA, and heterogeneous complex QA which require decomposed reasoning. We show that ICAT convincingly outperforms existing prompt-based solutions without involving any model training, showcasing the benefits of re-using existing abilities.

==> 01-introduction.tex <==
\section{Introduction}

\label{sec:intro}

% The advent of Large Language Models (LLMs) such as GPT-3~\cite{brown2020gpt3} and GPT-4~\cite{openai2023gpt4}, PaLM~\cite{chowdhery2022palm} have shown to significantly enhance understanding and generation capabilities for various language tasks~\cite{gpt3_prompting,gpt3incontext,ouyang2022training}. With increasing scale, these models 
% have demonstrated improved performance and sample efficiency on a range of tasks \cite{kaplan2020scaling}. These models also exhibit emergent capabilities such as few-shot in-context learning where few examples in form of (input, output) pairs are provided to the LLM to enunciate the intended task clearly. This has proved to be immensely effective for question-answering, particularly for complex QA tasks \cite{few_shot, self_ask}. 


% Complex Question Answering (QA) systems cater to precise information needs by performing latent reasoning and generating explanations for arriving at the solution. 

Answering complex questions is an active research topic that has widespread applications in finance, medical diagnosis, technical support, and more, enabling in-depth information access and advanced problem-solving~\cite{roy2022question:book}.
Complexity could arise from multiple factors, such as the need to parse heterogeneous sources \cite{chen2022finqa} or multiple documents \cite{tang-etal-2021-multi} to answer the question. 
It could also arise from the nature of the questions, such as compositional questions \cite{2wikimultihopqa, trivedi-etal-2022-musique}, which require reasoning through question decomposition to arrive at the final answer \cite{decomposing_complex_multi_hop} or numerical reasoning \cite{chen2022finqa,aqua_rat,roy2016solving}. 

An example of a compositional natural language question is \textit{``Who is the spouse of the person who voices Jarvis in Iron Man?"}. To answer this question, it must be first decomposed into relevant sub-questions, such as \textit{``Who voices Jarvis in Iron Man ?"} and \textit{``Who is the spouse of Paul Bettany?"}. To arrive at the final answer, a system must answer the sub-questions and aggregate their answers. The decomposition leads to interpretable reasoning apart from improved performance on the answering task. In numerical reasoning-based complex questions, stepwise decomposition of the reasoning process, usually called rationales, helps induce arithmetic abilities to arrive at the correct solution \cite{aqua_rat,roy2016solving}. 
Alternate approaches also involve generating arithmetic programs from the given natural language problem statement. \cite{chiang-chen-2019-semantically,amini-etal-2019-mathqa}. 

Existing methods for compositional complex QA adopt supervised \cite{decomposing_1, zhou-etal-2022-learning-decompose, min-etal-2019-multi,decomposing_complex_multi_hop, khot2021textmodular, deng2022interpretable} or unsupervised approaches \cite{perez-etal-2020-unsupervised} to decompose a complex question into simpler questions and provide the final answer by aggregating answers to the sub-questions. 
Similarly, numerical reasoning questions require supervised stepwise rationales along with the solution for fine-tuning generative models \cite{aqua_rat,cobbe2021training, geva-etal-2020-injecting}. More recently, LLMs have demonstrated impressive emergent capabilities to perform new tasks when provided with few-shot samples in the form of (input-output) pairs \cite{openai2023gpt4,chowdhery2022palm,few_shot,brown2020gpt3}. This emergent capability known as in-context learning \cite{gpt3_prompting,gpt3incontext,ouyang2022training,kaplan2020scaling} does not require time-consuming fine-tuning of models, but rather relies on the abilities of pre-trained LLMs to perform diverse tasks.

\mpara{The limitations of few-shot learning for complex QA.} The few-shot learning paradigm in LLMs alone does not prove to be sufficient to solve complex reasoning tasks such as numerical reasoning and complex multi-hop question answering \cite{rae2022scaling}. It is immensely hard for the LLMs to perform multi-step reasoning with aid of only parametric memory and the plain specification of (input, output) pairs due to limited information.

To solve complex QA tasks like numerical reasoning or compositional natural language questions, the LLMs are required to perform stepwise reasoning through decomposition, as discussed earlier. To induce such stepwise reasoning process in LLMs, Chain-Of-Thought (COT) prompting \cite{wei2023chainofthought} proposes to add hand-crafted natural language rationales to the prompts in addition to input and output (input, rationale, output). The process of generating stepwise natural language rationales can be seen as decomposing the original problem to simpler problems that can be solved with less effort. This has demonstrated impressive gains in numerical reasoning questions \cite{wei2023chainofthought, brown2020gpt3}.

Also, COT rationales for compositional natural language questions involve generating explanations for the final answer. However, such explanations have been found to be unfaithful to the reasoning process of underlying LLM \cite{turpin2023language,ye2022unreliability} for answering compositional questions in complex QA, unlike numerical reasoning questions. In such cases, the decomposition of such question to simpler sub-questions are observed to be more faithful. To induce such decomposition capabilities in LLMs, authors of the work self-ask \cite{self_ask} modify COT prompting and propose to add hand-crafted followup questions derived from the original complex questions to the prompt.

\mpara{The issues in manual In-Context COT construction.} We observe that the generation of natural language rationales for numerical reasoning and decomposition of complex multi-hop QA questions can be seen as \textbf{abilities} to be transferred to the LLM for downstream complex QA tasks. Existing approaches require careful hand annotated sub-questions or natural language rationales. This limits the information contained in exemplars, as it is cumbersome to hand-annotate a large pool of samples in the training set. Additionally, different tasks require the annotator to craft different reasoning chains, resulting in non-trivial efforts. Though approaches like \zfshot{} \cite{kojima2023large} have been proposed, they rely on the knowledge encoded in parameters of LLM without explicit demonstrations of the reasoning process, resulting in hallucinated steps and wrong solutions. Though it has been demonstrated to be a strong baseline for numerical reasoning, it is difficult to extend the method to tasks such as complex question answering, which require a more faithful decomposition when compared to rationales for numerical reasoning questions.


\mpara{\icat{} (In-Context Ability Transfer).} In this work, we propose a new approach for inducing stepwise decomposition abilities in LLMs for complex QA without costly fine-tuning or manual annotation processes. Our approach involves selecting  datasets named \transfer{} datasets which contain the desired ability required to solve a target task. For instance, to solve mathematical reasoning questions, reasoning stepwise through natural language rationales leads to better solutions \cite{wei2023chainofthought}. However, expert natural language rationales are not available for many datasets. Similarly, complex reasoning tasks require the ability to decompose complex questions. To induce this ability in LLMs, we propose to choose exemplars from related datasets with expert annotations for stepwise decomposition of complex questions or rationales for numerical reasoning. The list of \transfer{} and \target{} datasets and required abilities are shown in Table \ref{tab:transfer}.


% \subsection{Research Questions}

% We address the following research questions:

% \mpara{RQ1} Can we generate plausible decomposition or rationales for complex questions through~\icat{}, from~\transfer{} datasets ?

% \mpara{RQ2} Does the resulting decomposition help achieve competitive performance when compared to classical \COT{} approach for diverse, complex QA tasks?


% \mpara{RQ3} Does the proposed auto exemplar selection method improve performance of \icat{}?

\mpara{Contributions.} The core contributions of our work are:
\begin{description}
    \item 
    1) We propose a new approach ICAT that re-uses rationales from similar ability datasets for effective chain-of-thought reasoning.

    \item 
    2) We propose a novel uncertainty-aware exemplar selection approach for dynamic prompt construction that can achieve competitive performance with no manual intervention.
    
    \item 
    3) We conduct extensive experiments with different exemplar selection methods to showcase the generalized performance of ICAT across multiple complex QA tasks.
\end{description}

==> 02-related.tex <==
\section{Related Work}

% In this section, we briefly discuss the emergent capabilities in LLMs and the different In-Context learning paradigms adopted.


\subsection{Complex Question Answering and Question Decomposition}

Question Answering (QA) engines help cater to the precise information needs of users.
 The end-end QA systems that work well for single-hop QA datasets fall short in terms of performance and interpretability for compositional questions in multi-hop QA datasets \cite{multi_hop_survey,decomposing_complex_multi_hop}. 
 These end-end systems have unclear internal reasoning processes and the explanations from such systems are not faithful \cite{decomposing_complex_multi_hop}. 
 To overcome this bottleneck, several works have proposed supervised \cite{decomposing_1, zhou-etal-2022-learning-decompose, min-etal-2019-multi,decomposing_complex_multi_hop, khot2021textmodular, deng2022interpretable} and unsupervised approaches \cite{perez-etal-2020-unsupervised} to decompose a complex question into simpler questions and provide the final answer by aggregating answers to the sub-questions. 
 Prior works have also explored decomposing compositional questions to simple natural language queries \cite{decomposing_2_queries}. Patel et al. \cite{patel-etal-2022-question} demonstrated that manually decomposing complex questions to simpler sub-questions for LLMs provides better solutions.
% The Cambrian explosion of proprietary and open-source Large Language Models (LLMs) has resulted in widespread adoption for language tasks \cite{zhao2023survey} due to their enhanced generation and reasoning capabilities.  The performance of such LLMs on a range of tasks increase with rise in scale \cite{kaplan2020scaling, rae2022scaling,chowdhery2022palm}. It also leads to other characteristics such as sample efficiency. it has also been observed that with changes in scale, the larger models demonstrate new capabilities not observed in smaller scale models. These capabilities are termed \textit{emergent capabilities}, where the smaller models demonstrate near random performance on new tasks, but have a sharp raise in performance with increase in scale in terms of model parameters and pre-training data \cite{wei2022emergent}. Some of these emergent capabilities involve few-shot in-context learning, where the LLM is first given a few labeled input-output pairs as demonstration for performing a task. Then the model is given an unseen sample to perform an intended task. The LLM demonstrates the capability to infer and perform the task from few exemplars provided \cite{few_shot,shin-etal-2020-autoprompt}, without any gradient updates. For complex reasoning tasks like numerical reasoning, multi-step reasoning \cite{multi_hop_survey} few-shot prompting falls short when compared to existing approaches. This is due to the reliance on the parametric memory of the pre-trained LLM and limited task information presented in the  demonstration samples. 

% \begin{figure}
%     \includegraphics[width=\linewidth]{WSDM_2024/figures/schematic-icat.pdf}
% \end{figure}

\subsection{Chain of Thought for Complex Question Answering}

To solve complex tasks like numerical reasoning and complex QA, multi-step reasoning helps improve overall performance. Prior work in numerical reasoning \cite{aqua_rat,cobbe2021training}, have demonstrated that stepwise rationales for arriving at the final solution helps to arrive at more accurate solutions. However, these approaches are expensive in that they require expert annotated rationales for fine-tuning a model to generate rationales at inference time. Though few-shot ICL \cite{few_shot,shin-etal-2020-autoprompt} of LLMs have demonstrated impressive performance in many tasks, they do not perform well for complex reasoning tasks \cite{rae2022scaling}. To augment more information in the exemplars provided for ICL, prior works \cite{wei2023chainofthought,lewkowycz2022solving} have proposed hand annotated stepwise rationales (Chain of Thought) for arriving at the solution for numerical reasoning problems. Additionally, the zero-shot \cite{kojima2023large} generation of such rationales through simple prompt engineering without demonstrations serves as a strong baseline across datasets.


In a  similar manner, complex QA tasks usually require multi-step reasoning \cite{yang-etal-2018-hotpotqa,strategy_qa, trivedi-etal-2022-musique,2wikimultihopqa} to solve different types of questions like compositional, bridge and comparison questions. Chain of thought prompting \cite{wei2023chainofthought} for complex QA involves generating an explanation for the answer to the question. However, studies have indicated that such explanations are unfaithful \cite{turpin2023language} to the model's reasoning process and the model ignores the COT explanation at times when arriving at the final answer. Alternate approaches like successive prompting \cite{dua-etal-2022-successive} proposes to generate a sub-question followed by another call to answer the question. This leads to a computationally expensive inference phase. To arrive at a concise answer in a stepwise manner, self-ask \cite{self_ask} proposes decomposing compositional questions to simpler follow-up questions but requires hand-crafted demonstration samples. Further, inspired by retrieval augmented LLMs\cite{khandelwal2020generalization,lewis2021retrievalaugmented}, self-ask combines neural LMs with search for arriving at more accurate answers for sub-questions. 

However, a major drawback in proposed approaches is the need for manual annotation of rationales or sub-questions. This is cumbersome and also limits the generality of the approach, as the chosen exemplar pool is limited to annotated samples. In this paper, we focus on transferring the ability to generate rationales for numerical reasoning and ability to decompose complex questions. We accomplish this by relying on \transfer{} datasets with expert annotated rationales or sub-questions.

Our work is also inspired by the theory of LLMs performing Bayesian inference \cite{xie2022explanation}. The authors argue that In-Context learning helps learn a distinguishable concept. Our proposal to transfer abilities is similar in spirit to this theoretical framework.

\subsection{Exemplar  Selection for ICL}

Though random or manual selection of demonstration samples (exemplars) for ICL have demonstrated impressive performance, they have several limitations. The designed prompts have shown to affect performance by being sensitive to order, dataset, task, and models \cite{zhao2021calibrate,su2022selective, lu-etal-2022-fantastically}. Prompt engineering is still an ongoing effort as it is a complex multi-objective optimization problem to select few empirical observations for achieving stable performance on wide range of test samples. Few auto exemplar selection methods like similarity based \cite{rubin-etal-2022-learning} approaches, complexity based \cite{complex_cot} and MMR \cite{ye-etal-2023-complementary} based approaches for diverse example selection have been proposed to achieve stable performance across wide range of tasks. However, for COT dynamic retrieval of exemplars for each test sample requires annotations of rationales/reasoning paths for the whole training set which is cumbersome. Though Auto-COT \cite{zhang2023automatic} proposes to mitigate manual annotation, it relies on zero-shot-cot for designing exemplars which is erroneous and leads to error propagation on downstream questions. Hence, in our work, we study existing auto selection methods in a novel setting where we select exemplars from transfer datasets with expert rationale annotations. We also propose a new exemplar selection method and evaluate it's effectiveness across a wide range of tasks.

==> 05-experiments.tex <==
\input{table-datasets}

\section{Experiments}
\label{sec:experiments}
In this section, we describe the experimental setup to answer the research questions in Section \ref{sec:intro}.

% \mpara{RQ1} Can we generate plausible reasoning steps for complex reasoning tasks through the ability transfer paradigm \icat{}, from transfer datasets ?

% \mpara{RQ2} Does the transferred abilities achieve competitive performance when compared to classical few-shot COT approach for diverse complex reasoning tasks?


% \mpara{RQ3} Does auto exemplar selection methods improve performance of \icat{} paradigm ?


\subsection{Datasets}

We focus our experiments on tasks of numerical reasoning and complex compositional multi-hop QA. We evaluate on Multiarith \cite{roy2016solving}, SVAMP \cite{patel2021nlp}, 2WikimultihopQA (WQA) \cite{2wikimultihopqa} and MusiqueQA (MQA) \cite{trivedi-etal-2022-musique}. We evaluate on test sets of Multiarith and SVAMP. For WQA, we sample 1200 questions from validation sets following works such as self-ask \cite{self_ask} for a fair comparison. For MQA we evaluate on the 1252 two-hop questions.

To also showcase the ability of \icat{} to transfer in heterogeneous settings, we transfer the ability to generate rationales from datasets like AQUA-RAT or TABMWP to the LLM for evaluation on the target dataset FinQA. We term this Ability transfer for heterogeneous settings as AQUA-RAT contains only plain math word problems and TABMWP is table based numerical reasoning. However, finQA requires reasoning over table and text to solve the problem.

\subsection{Setup}

All our experiments are primarily carried out with instruction fine-tuned LLMs like \textit{gpt-3.5-turbo} unless otherwise specified. 
For all experiments, we set the temperature to $0.3$ to mitigate randomness, with frequency and presence penalty set to 0.8 and $0.6$ to avoid repetition. 
We cap the max For all datasets, we use k=6 for all auto-exemplar selection methods. For MMR, we experiment with various values of $\lambda$ and observe $0.7$ to be the best value based on evaluations on a small split of train set. For WQA dataset, we use multiple transfer sources, since the questions are compositional in nature and also contain comparison questions. We transfer exemplars from both SubQA and StrategyQA as StrategyQA contains decomposition for comparison questions. We select 4 exemplars from SubQA \cite{min-etal-2019-multi} and 2 from StrategyQA in this setting.

For static exemplar selection in the \ \icat{} vanilla approach, we carefully design heuristics to ensure the exemplars are diverse in that they cover different categories of questions asked in numerical reasoning and complex QA. For numerical reasoning we choose 6 exemplars from AQUA-RAT such that they cover different operators such as addition, multiplication, division and also exemplars which require compositional reasoning. 
The examples are shown in Table \ref{tab:datasets_overview}.
For complex QA datasets like WQA we choose exemplars that cover different categories namely \textit{compositional, comparison and inference}. Since questions in WQA encompass all the mentioned categories we transfer from both datasets namely SubQA \cite{tang-etal-2021-multi} and StrategyQA \cite{strategy_qa} ensuring the exemplars cover comparison, compositional and comparison type questions. Since MusiqueQA is primarily compositional, we transfer only from SubQA.


\subsection{Metrics}

For numerical reasoning, we report accuracy/exact match. For complex QA datasets WQA and MQA we report cover-EM \cite{cover_em, self_ask}.

\subsection{Baselines}

Some common prompting approaches we evaluate against are:

\textbf{Few-shot-COT}: We follow the hand annotated examples provided in prior works \cite{wei2023chainofthought, self_ask} as exemplars for ICL. For numerical reasoning this involves hand annotated step-by-step reasoning chains and for complex QA the annotations are in the form of explanations to arrive at the final answer. The manual annotation limits the choice of examples and is also cumbersome.

\textbf{Zero-shot-cot}: The zero-shot chain of thought introduced by \cite{kojima2023large} serves as a strong baseline across different tasks. This approach follows a simple prompt prefix \textit{``Let's think step by step"} to induce reasoning abilities in LLMs. 

We also use \fshot{} prompting \cite{brown2020gpt3} as baseline which does not involve reasoning chains.

\subsubsection{Numerical Reasoning}
\textbf{Auto-COT \cite{zhang2023automatic}}: In this approach, for each test sample, related questions are selected from the test set based on clusters formed. This is followed by zero-shot prompting to generate Chain of thought from a LLM. The exemplars are augmented with the generated COT and are used as prompts. An issue is propagation of errors from zero-shot COT outputs. Additionally, in complex QA the generated zero-shot explanations may not be faithful to the model.
\subsubsection{Complex QA}
\mpara{Self-ask} \cite{self_ask}: The recently proposed prompting approach for compositional QA. It involves manual, hand-crafted follow-up question annotations for a given question.
\subsubsection{Auto Exemplar Selection} 


\mpara{KNN} \cite{rubin-etal-2022-learning}: We first utilize the k-nearest neighbours based function to select exemplars from transfer dataset. First the sentence transformer based vector representations are computed for the training samples in $D_s$ and are stored in an index. At inference time for each $x_i^t \in D_t$ we retrieve top-k similar exemplars from the transfer data store. \ $S_{D_s} = top_k (Sim(x_i^s,D_s))$ 

\mpara{MMR} \cite{ye-etal-2023-complementary}: To induce diversity in the selected exemplars, the Maximum Marginal Relevance commonly used in IR \cite{carbonell1998use} is employed to select exemplar instances similar to $x_i^s$ but diverse with respect to exemplars already selected in set $S_{D_s}$ 
\[u^{s*} = \argmax_{u_i^s \in D_s \setminus S_{D_s}} \lambda Sim(x_i^t,u_i^s) - (1-\lambda) max_{u_j^s \in S_{D_s}} (Sim(u_i^s,u_j^s))\]
where $u_i^s = (x_i^s,y_i^s,z_i^s)$

\mpara{Random}: We also consider the scenario of random exemplar selection. We consider two cases, namely the static random and dynamic random, where the exemplars are selected once and for the latter case on a per-instance basis respectively.

==> 06-results.tex <==
\section{Results}
\label{sec:results}
\input{table_results}

We evaluate the proposed ability transfer approach \icat{} on the tasks of numerical reasoning and complex Question Answering to answer RQ I and RQ II. As discussed, our goal to transfer the abilities to generate rationales for numerical reasoning and to decompose complex questions to simpler sub-questions. We also demonstrate the ability to transfer to target datasets with heterogeneous sources like FinQA which requires numerical reasoning over table and text.

From the Table \ref{tab:main_result}, we observe that across tasks, the proposed \icat{} paradigm outperforms or achieves competitive performance with Few-shot Chain of thought approach or other task specific in-context learning methods. Our goal is not to beat the state-of-the-art, but to employ an efficient reasoning process without the overhead of manual annotations. We posit that this can be achieved through transferring required abilities from expert datasets from related or different domains.

\subsection{Performance on numerical reasoning tasks}
The Exact mach (EM) scores for multiarith and SVAMP numerical reasoning datasets are shown in Table \ref{tab:main_result}. We observe that the proposed approach \icat{} with the static, but careful selection of exemplars outperforms the zero-shot-cot baseline. We observe that this is because the model hallucinates reasoning and final solution in zero-shot-COT due to lack of demonstrations.

We also observe that \icat{} (static) performance is competitive or outperforms manual few-shot chain of thought (\COT{})\cite{wei2023chainofthought}. This demonstrates that careful and manual selection of exemplars from transfer datasets that cover diverse categories of questions are sufficient for generating good rationales and downstream problem-solving task. We also observe gains over Auto-COT \cite{zhang2023automatic}, a more recent approach to generate rationales for chosen exemplars by using zero-shot-COT. We observe that though Auto-COT is close to performance of manual \COT{}, the decline in performance is due to mistakes in rationales generated through zero-shot-COT. For instance, for a question

\mpara{Q:}\texttt{ 5 children were riding on the bus. At the bus stop, 63 children got off the bus. Then there were 14 children. How many more children got on the bus than those that got off?} 

generated rationale is \textit{``Rationale: Let's think step by step. There were 63 children that got off the bus. That means there were 68 children on the bus before the 63 got off. 14 children remained on the bus, which means 54 children got on the bus. Therefore, 54 - 63 = -9. 9 more children got on the bus than those that got off. The answer is 9"}

Though the answer is correct the rationale is wrong as the operation should be ``14-9". This shows that the rationale is not necessarily faithful in zero-shot-COT and may contain errors in reasoning.

We also evaluate auto-exemplar selection methods. Note that this is different from classical selection methods in few-shot prompting, as our goal is to select exemplars from transfer datasets which are from a different distribution than the test example. Also, the exemplars are annotated with expert rationales which enable to select few-shot examples with rationales unlike manual \COT{}, where randomly chosen samples are manually annotated with rationales limiting the pool to select samples from. We observe that the proposed uncertainty-aware term embedding distribution based metric \textit{\ftd{}} offers more stable performance across SVAMP (\textbf{80.7 \%}) and multiarith and is competitive or offers gains over existing auto-exemplar selection approaches like KNN or MMR and is better than random selection approaches. We observe that our careful manual selection of exemplars (\textit{\icat{} (static)}) is competitive or slightly underperforms compared to auto-exemplar selection methods. This is inline with the observation made in the work \cite{zhou-etal-2023-revisiting} that careful manual selection of exemplars are competitive with automated selection. However, auto-exemplar based selection methods are more stable to minor perturbations in order, dataset and models \cite{zhao2021calibrate,su2022selective, lu-etal-2022-fantastically}. We observed that \icat{} (\ftd{}) in general selected representative and diverse samples that covered different categories of numerical reasoning problems which might have positively contributed to the rationale and solution for the test problem. However, we posit that more structured prompting methods that exploit the algebraic operator tree might aid in better exemplar retrieval. Since dense representations favor thematic similarity more, they may not directly optimize for selecting exemplars with similar math expression as the test example. We plan to explore this direction of structure aware prompting in the future.  
%\sourangshu{Need more experiments here probably to show stability on our datasets}.

\mpara{Insight 1:} \textit{\icat{} approach performs well in numerical reasoning, particularly on questions requiring compositional reasoning (multiple arithmetic operations).}

\subsection{Performance on complex QA reasoning tasks}
For complex QA task we evaluate on 2WikiMultiHopQa (WQA) and MusiqueQA (MQA) and the results are tabulated in Table \ref{tab:main_result}. Here the complexity arises from the need to do compositional multi-hop reasoning or from comparison questions. We observe that \icat{} (static) offers competitive performance with Few-shot-COT and  state-of-the-art methods like self-ask on WQA and outperforms existing approaches on MQA. We observe that on WQA we are able to achieve competitive performance only when transferring from both SubQA and StrategyQA and the performance drops when transferring only from either of the datasets. We observe that the performance of \COT{} is not consistent across MQA and WQA as it underperforms on MQA. This is primarily because \COT{} for complex QA generates an explanation to arrive at the final answer without any question decomposition. This is sometimes observed to be unfaithful to the model reasoning process \cite{turpin2023language} and hence can be plausible but misleading. We also observe that at times the rationales generate factually inconsistent explanations, resulting in an incorrect answer, as shown in table \ref{tab:qualitative}. It has been observed that question decomposition is faithful to model reasoning process \cite{decomposing_complex_multi_hop} and also generates simpler sub-questions for reasoning. We attribute the performance of \icat{} (static) and  \icat{} + (\ftd{}) to this observation, as the transfer datasets contain expert annotated sub-questions.

Among auto-exemplar selection approaches, we observe that the proposed \ftd{} based exemplar selection (\icat{} + (\ftd{})) outperforms static selection and random selection. It also outperforms exemplar selection  methods like KNN and MMR on WQA dataset and offers slight gains on MQA dataset. We observe that the results from \ftd{} are more consistent and stable compared to other auto-exemplar selection methods or static selection methods across datasets. We attribute this to the ability of FTD to select high-quality and diverse exemplars, ensuring global consistency \cite{frechet_language} from transfer datasets based on term distribution distance between the test sample and candidates in transfer datasets. Whereas, \knn{} and \mmr{} rely on local surface level characteristics of the instances. On examining the selected exemplars from \ftd{}, we observe that they matched the thematic style (location based, temporal questions etc..) of the test question and also the type of question (\textit{compositional, comparison}). Hence, we posit that representative, diverse exemplars with high quality annotation of reasoning steps like rationales or sub-questions induce faithful reasoning in LLMs for new questions. \ftd{} is also less sensitive to choice of embedding model \cite{frechet_language}, unlike \knn{} and \mmr{}.

\mpara{Insight 2:} \textit{Question decomposition through manual or automated exemplar selection from transfer datasets is more faithful to model reasoning process than \COT{}. The choice of representative exemplars and the quality of the sub-questions are critical to downstream performance on complex QA datasets. }

\subsection{Performance on Heterogenous Ability Transfer}
% \input{prompt_finQA}
\input{table-qualitative}

\begin{figure}
     \begin{subfigure}[b]{0.2\textwidth}
         \includegraphics[width=\textwidth]{figures/musique.pdf}
         \label{fig:y equals x}
     \end{subfigure}
     %\hspace{-3em}   
     \begin{subfigure}[b]{0.2\textwidth}
         
         \includegraphics[width=\textwidth]{figures/finQA.pdf}
         \label{fig:three sin x}
     \end{subfigure}
     \vspace{-1em}   

     % \begin{subfigure}[b]{0.2\textwidth}
     %     \includegraphics[width=\textwidth]{figures/multiarith.pdf}
     %     \label{fig:five over x}
     % \end{subfigure}
        \caption{Confusion matrices across tasks comparing \icat{} vs \COT{}}
        \label{fig:conf_matrix}
\end{figure}

One of the important conditions for the proposal \icat{} paradigm is for the need of expert annotated rationales/decomposition in tasks which are related to the target task. However, several target tasks may require abilities from other tasks, which may not be necessarily related. For instance, complex claim verification tasks like CLAIMDECOMP \cite{claimdecomp} may benefit from generating sub-questions for evidence retrieval. This ability to generate sub-questions could be transferred from expert annotated sub-questions in SubQA. Similarly, heterogenous (table and text) numerical reasoning tasks like FinQA \cite{chen2022finqa} may benefit from natural language rationales deriving the solution in a  stepwise manner. To explore if it is possible to transfer abilities across tasks with different characteristics, we test the ability to transfer the ability to generate rationales from AQUA-RAT and TABMWP to FinQA. The results are shown in Table \ref{tab:main_result}. We observe that transferring from AQUA-RAT achieves decent performance, but still underperforms when compared to Few-shot-COT. This is because of the homogeneous setting of AQUA-RAT, which involves numerical reasoning based on text. However, FinQA requires reasoning over table and text, and we observe that the ability to parse table information to retrieve the appropriate numerical quantities are critical to the task. We observe that when \icat{} attempts to transfer the rationale generation ability based on few-shot examples from AQUA-RAT it results in erroneous rationales due to accessing wrong information in tables. To induce the ability to parse tables in a few-shot setting, we apply \icat{} to transfer ability to parse tables and generate rationales from TabMWP \cite{lu2023dynamic} a table based reasoning dataset. We would like to point out that this still accounts for heterogeneous transfer, as the target task is focused on transferring from both table and text. We observe that \icat{} (TabMWP) offers gains over existing approaches and also slight gains over Few-shot-COT. This supports our hypothesis that transferring the ability to parse tables along with rationale generation is critical to the FinQA target task. An example of a FinQA question is shown in Table \ref{tab:qualitative}. We observe that it is a compositional heterogeneous numerical reasoning question which requires decomposed reasoning for different time periods and aggregation of answers. This requires parsing the correct information regarding securities and brokerages for 2009 and 2010 from table and text and adding them up to arrive at the final answer. We observe that the Few-shot-COT prompts provided in \cite{chen2022program} are not detailed enough, in that they do not spell out the fields to access for information and also do not contain the algebraic expression to arrive at the final answer as shown in Figure \ref{fig:incontext}. However, in Figure \ref{fig:incontext}, we observe that the exemplars selected from TabMWP by \icat{} details the fields to access for the required information to solve the problem in the form of expert annotated rationale followed by the final algebraic expression to arrive at the solution. TabMWP is pre-annotated with expert rationales and hence obviates need for manual annotation like Few-shot-COT.
Hence, we posit that in lack of similar tasks for transfer, datasets that contain desired abilities to solve parts of the task are still useful in a few-shot ICL setting.

\mpara{Insight3}: \textit{ \icat{} works well for transfer to heterogeneous tasks by selecting specific abilities from candidate examples in transfer datasets to solve parts of target task.}



\subsection{Impact of the different LLMs employed}
We also evaluate the proposed approach \icat{} using open-source models like \flan{} (0.8B) and \flanxl{} (3B) to study the impact of scale and other properties of LLMs employed. We observe from table \ref{tab:main_result} that scale of the LLM is critical apart from instruction based pre-training. This is due to the emergent capabilities being more pronounced in models of higher parameter scales \cite{wei2022emergent}. We also observe that apart from scale, models trained with high quality instructions perform better at diverse reasoning tasks. This is evident from \icat{} with gpt-3.5-turbo as backbone outperforming text-davinci-003 as shown in Table \ref{tab:main_result}.
\subsection{Qualitative Analysis}

We perform a qualitative analysis across datasets by randomly sampling 150 samples from evaluation sets of each dataset. We also plot the confusion matrices for the full evaluation sets for \icat{} vs \COT{}, as shown in Figure \ref{fig:conf_matrix}. For numerical reasoning datasets MultiArith and SVAMP, we observe that \icat{} performs well on compositional reasoning, which requires performing multiple dependent arithmetic operations. We observe that in most of the erroneous instances in output of \COT{}, the questions are of compositional nature which require multistep arithmetic reasoning. On inspection, the rationale reveals that the reasoning is incomplete where the LLM only outputs part of the operation as it is unable to infer all the operations to be performed. We make a similar observation for FinQA as demonstrated by the example in Table \ref{tab:qualitative}. We observe that the \COT{} does not take the securities information into account and misses performing addition of these values. However, \icat{} and \icat{} + \ftd{} are able to arrive at the correct answer due to the quality of rationales in the \transfer{} dataset TabMWP. Similarly, on compositional complex QA, we observe that \icat{} produces a decomposition that is faithful to the LLM reasoning process whereas \COT{} provides a rationale which results in hallucinated, incomplete  or unfaithful responses. Examples from WQA and MusiqueQA (MQA) are shown in Table \ref{tab:qualitative}. We observe that the first example hallucinates \textit{``Julia Andrews"} as the answer, whereas the faithful decomposition by \icat{} results in the correct answer. Similarly, in the second example in the table we observe that \COT{} is unable to retrieve the birthdate of ``Holm Jolsen" from parametric memory, whereas our approach is able to correctly retrieve the answer followed by a comparison step to arrive at the correct answer.

\section{Conclusion}
%\input{table-errors}

% \sourangshu{(notes:\\
% EM: Exact Match accuracy\\
% Table 1: Numerical reasoning (SVAMP, MultiArith)\\
% Table 2: Multihop QA (2WikiMHQA, MusiqueQA) \\
% Table 3: FinQA \\
% ICAT(static) - hand picked demonstration samples\\
% ICAT(random) - randomly picked demonstration samples for each test sample\\
% ICAT(KNN) - k-nearest neighbors to the test sample according to sentenceBert encoding used as demonstration samples\\
% ICAR(MMR) - k-highest neighbors selected according to MMR objective which balances selectivity with diversity.}

==> abstract.tex <==
Question Answering (QA) systems cater to the precise information needs of the user. However, complex questions that are compositional in nature require multistep reasoning for arriving at the solution, along with explanatory rationales  to demonstrate the reasoning process. However, this is a challenging task with limited or no supervision available for the reasoning/decomposition process. Recent advances in Large Language Models (LLMs) have led to their deployment in answering complex questions through few-shot demonstration of exemplars with manually annotated rationales or reasoning steps to arrive at the final answer. Though this approach leverages the emergent capabilities like in-context learning in LLMs, the collection of reasoning steps like the rationales or the decomposed sub-questions are cumbersome as they are hand annotated. Motivated by the scarcity of annotated reasoning steps, we propose, \icat{} (In-Context Ability Transfer) which induces reasoning capabilities in LLMs without any LLM fine-tuning or manual annotation of in-context samples. We transfer the ability to decompose complex questions to simpler questions or generate step-by-step rationales to LLMs, by careful orchestration of data subset selection from available data sources of related tasks. These data sources house examples with annotated reasoning steps and are from a different distribution than the target tasks. We evaluate \icat{} on diverse tasks of numerical reasoning, compositional complex QA and heterogeneous complex QA which require decomposed reasoning. We also propose an automated uncertainty-aware exemplar selection approach for selecting examples from \transfer{} data sources.

% Large Language Models (LLMs) have demonstrated impressive capabilities and are widely adopted for NLP and IR tasks. These models demonstrate emergent abilities where they are able to perform complex reasoning tasks through exemplars provided as in-context samples. However, several works have demonstrated that the performance of LLMs largely depends on selection of these examples and manual stepwise rationale annotations for such examples becomes cumbersome with an increase in number of samples provided. Though zero shot reasoning is an alternative, it limits the reasoning capabilities of LLMs due to the lack of required information, resulting in hallucinated outputs. Motivated by the scarcity of annotated reasoning steps for complex reasoning tasks, we propose a new data-centric paradigm where the stepwise decomposition process for reasoning is transferred from other relevant data sources with expert annotated reasoning steps. We propose a new paradigm named In-Context Ability Transfer (ICAT) which induces reasoning capabilities in LLMs without any LLM fine-tuning or manual labeling of in-context samples by careful orchestration of data subset selection from available data sources. We evaluate this paradigm in the context of decomposition for numerical reasoning and multi-hop question answering. We demonstrate that the proposed paradigm achieves competitive performance to existing approaches without manual annotation. We also propose a term distribution distance based automated exemplar selection method for achieving stable results.

==> intro-example.tex <==
\begin{table}[t]
\center
% \small
% \makegapedcells
\begin{tabular}{lll}
\toprule
\multicolumn{3}{l}{\texttt{What did the actress in My Fair Lady win a Tony for?}}             \\
                 \midrule
\textsc{COT} & \textcolor{magenta}{\textsc{The actress in My Fair Lady is Julie Andrews}}     & She won the Tony for the best actress \\

Correct          & \textcolor{teal}{\texttt{Schindler's List}} &F.G. won Oscars in \textbf{1995}    \\
\midrule
\\
                \multicolumn{3}{l}{\makecell[l]{\texttt{Who lost the WBA boxing title, refusing to fight Tony } \\ \texttt{Tucker in March 1995?}}}      \\
                 \midrule
\textsc{Alpaca}  & \textcolor{magenta}{\texttt{Mike Tyson}}       & \xmark{} \textit{Popularity bias:}        \\
Correct          & \textcolor{teal}{\texttt{George Foreman}}   &   time disregarded \\
\midrule
\\
                  \multicolumn{3}{l}{\texttt{Tom Brady played for which team in 2020?}} \\
                 \midrule
\textsc{Alpaca}  & \textcolor{magenta}{\texttt{New England Patriots}} & \xmark{} \textit{Temporal Inertia}: Brady   \\

Correct          & \textcolor{teal}{\texttt{Tampa Bay Buccaneers}} &  joined Buccaneers in 2020   \\
\bottomrule
\end{tabular}
\caption{Examples of temporal blindspots in LLMs. }
\label{tab:intro_example}
\end{table}

==> prompt_finQA.tex <==
\begin{table}[hbt!]
% \scriptsize
\Small
\begin{tabular}{p{8cm}}
\toprule 
\textbf{Prompt FinQA:}
% \midrule
\\
\midrule

% I am a highly intelligent question answering bot. If you ask me a question that is  \\
%   rooted in truth, I will give you the answer. If you ask me a question that is  \\  
%  nonsense, trickery, or has no clear answer, I will respond with 'Unknown'.\\ \\ 


 
\texttt{Few-shot-COT (exemplars from FinQA) \cite{chen2022program}} \\ Text: annual sales of printing papers and graphic arts \\supplies and equipment totaled \$ 3.5 billion in 2012 compared with \$ 4.0 billion in 2011...
\\
\textbf{Table}: in millions | 2012 | 2011 | 2010 \\
sales | $ 6040 | $ 6630 | \$ 6735 \\
operating profit | 22 | 34 | 78 \\
\textbf{Question}: what percent of distribution sales where \\attributable to printing papers and graphic arts supplies and equipment in 2011?\\
\textbf{Rationale}: The sales of print papers and graphic arts \\ supplies and equipment in 2011 is 3.5 billion. The 
 \\ total sales in 2011 is 6.63 billion. The percentage is 52.8\%. So the answer is 52.8\%. \\
Answer:52.8%
\\ \\ 

\texttt{\icat{} (Transfer from TabMWP)} \\                           \textbf{Question}: A stock broker followed the \\stock prices of a certain set of companies. How much more did Thompson Corporation's stock cost on Monday than on Tuesday?,
\\
\textbf{Table}: Company | Monday | Tuesday
White and Company | \$11 | \$17 \\
Thompson Corporation | \$16 | \$9
\\ Watson and Partners | \$1 | \$16
\\ Houston Sporting Goods | \$15 | \$7
\\Computer Data Company | \$4 | \$20
\\
\textbf{Rationale}: Find the Thompson Corporation row.  Find the numbers in this row for Monday and Tuesday.\\Monday: \$16.00 Tuesday: \$9.00  Now subtract:\$16.00 - \$9.00 = \$7.00
Thompson Corporation's stock cost \$7 more on Monday than on Tuesday.
\\ \textbf{Answer}: 7

\\ \\ 



\bottomrule
\end{tabular}
\caption{Example of In-context learning through manual few-shot-COT prompting and \icat{} based prompting of LLMs (limited examples shown)}
 \label{fig:incontext}
\end{table}

==> table-errors.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{p{4cm}|p{5cm}|p{2cm}}
         \textbf{Question} & \textbf{Reasoning path} & \textbf{Error Type}  \\ \hline
         & & \\ \hline
         & & \\ \hline
        
    \end{tabular}
    \caption{Analysis of errors on complex QA tasks.}
    \label{tab:my_label}
\end{table*}

==> table-transfer.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|p{1.8cm}|p{2.2cm}|p{0.7cm}|p{2.7cm}|}
       \textbf{Transfer}  & \textbf{Target} & \textbf{JS} & \textbf{ Transfer Ability}\\ \hline
         AQUA-RAT & MultiArith & 0.364 &Rationale generation  \\       

        AQUA-RAT & SVAMP & 0.379 & Rationale generation\\ \hline

        SubQA, StrategyQA  &2WikiMultiHopQA & 0.335, 0.573 & Question decomposition, Implied sub-questions \\
         
SubQA & MusiqueQA & 0.236 & Question decomposition
         \\ \hline
TabMWP & FinQA & 0.388 & Rationale generation for Table and Text based numerical reasoning, Parsing tables
\\ \hline
    \end{tabular}
    \caption{\transfer{} datasets and \target{} datasets.}
    \label{tab:transfer}
\end{table}

==> table_results.tex <==
\begin{table*}[!t]
    \centering
    
    \begin{tabular}{llccccc}
    \toprule
     &\multirow{2}{*}{Method}& \multicolumn{1}{c}{MQA}& \multicolumn{1}{c}{WQA} & \multicolumn{1}{c}{MultiArith} & \multicolumn{1}{c}{SVAMP}& \multicolumn{1}{c}{FinQA}\\
     && cover-EM & cover-EM& EM& EM&EM \\
     \midrule
     \multirow{5}{*}{\textbf{Baselines}}&\fshot{} \cite{brown2020gpt3}& 11.66& 28.41& 85.74& 78.2& 42.55\\
     &\COT{} \cite{wei2023chainofthought}&20.85& 34.08&94.79&  79.4&52.22 \\
     &\zfshot{} \cite{kojima2023large}& 12.22& 19.25& 88.75& 75.4& 47.51 \\
    &\self{} \cite{self_ask}& 23.64& 32.58& N/A& N/A& N/A \\
      &\autocot{} \cite{zhang2023automatic}&  N/A& N/A&  93.83 & 76.2 & N/A \\
     \midrule

      \multirow{2}{*}{\textbf{\icat{} (ours)}}
               &text-davinci (static) &  20.28& 25.33&  81.71 & 74.7 & 40.01 \\
    &\flan{} (static)&  1.59 & 20.00 &  10.25 & 8.31 & 1.48 \\
          &static random&  23.24& 25.08&  92.44 & 75.90 & 51.17 \\
      &\flanxl{} (static)&  2.96 & 17.92 &  24.48 & 22.08 & 1.92 \\&static &  25.24& 34.00&  96.14 & 80.0 & 53.35 \\



      \midrule
    \multirow{5}{*}{\textbf{\icat{} (ours) (auto,dynamic)}}
     
      &random&  24.36& 29.41&  92.95 &   77.60 & 50.74 \\

    &\knn{}  &  26.99& 30.69&  95.13 & 80.70 & 52.65 \\
     &\mmr{}  &  27.07& 30.33&  94.96 & 80.70 & 52.14 \\
       &\ftd{} &  \textbf{27.24}$\ddagger$& \textbf{36.00}&  \textbf{96.14}$\dagger$ & \textbf{80.70} & \textbf{55.36}$\dagger$ \\
     \bottomrule
    \end{tabular}
    \caption{Results across datasets. The model used for \icat{} and other SOTA few-shot prompting based approaches is gpt-3.5-turbo unless otherwise specified.$\dagger$ and $\ddagger$ indicates statistical significance over \COT{} at 0.1 level  and 0.01 level respectively.}
    \label{tab:main_result}
\end{table*}


\begin{table}[!t]
    
    
    \begin{tabular}{p{1.3cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{1cm}}
    \toprule
     &\multirow{2}{*}{Method}& MQA& WQA & MA & SV& FinQA\\
     && C-EM & C-EM& EM& EM&EM \\
     \midrule
     \multirow{1}{*}{\textbf{supervised}}
     % &FinQaNET (FinBERT) & N/A& N/A& N/A& N/A& 50.10\\
     % &FinQaNET (RoBERTa-large) & N/A& N/A& N/A& N/A& 58.86\\
     % &Retriever +NeRd (BERT-base) & N/A& N/A& N/A& N/A& 48.57\\
     % &FiD & 37.6& 76.9& N/A& N/A& N/A\\
     % &Retriever +NeRd (BERT-base) & N/A& N/A& N/A& N/A& 48.57\\
     % &\zfshot{} \cite{kojima2023large}& 12.22& 19.25& 88.75& 75.4& 47.51 \\
     & SOTA & \bf 37.60  & \bf 50.59 &  60.5  &  47.3 & \bf 58.86\\
     \midrule
     \multirow{1}{*}
     {\textbf{\icat{}}} &\ftd{} (ours)&  27.24& 36.00& \bf 96.14 & \bf 80.70 & 55.27 \\
     \bottomrule
     \end{tabular}
     \caption{Comparison of \icat{} and existing SOTA supervised baselines across datasets, MA- MultiArith, SV-SVAMP}
     \end{table}
% \begin{table}[hbt!]
% \begin{tabular}{l|p{1cm}|p{0.8cm}|}

% \textbf{Method} & \textbf{EM(MA)} & \textbf{EM(SV)} \\\hline\hline

% \COT{} (PALM (540 B))                                 & 94.7                                    & 79.0                               \\
% \zfshot{}  (PALM (540 B))                                      & 66.1   & 69.4                               \\
% \COT{} (LAMDA (135 B))                                       & 51.8                                    & 57.9                     \\ \hline
%  % Zero-shot-cot (GPT3 (text-davinci))               & 72.99                                   & 63.7                               \\

% \zfshot{}  \cite{kojima2023large}                & 88.75                                   & 75.4 \\      
% \fshot{}     \cite{brown2020gpt3}                  & 85.74                                   &   78.2                                                        \\
% Auto-COT \cite{zhang2023automatic} & 93.83 &76.2 \\
% \COT{} \cite{wei2023chainofthought}                   & 94.79                                   &  79.4                                  \\\hline
% \icat{} (text-davinci) (ours)        & 81.71                                   & 74.7                               \\ 
% \icat{} (\flanxl{}) (ours)        & 24.48                                   &       22.08                         \\ \hline

% \icat{} (static) (ours)  & \textbf{96.14}$\dagger$                         &   80.0              \\

% \icat{} (static random) (ours)  & 92.44                        &        75.90             \\

% \icat{} + random (ours) & 92.95                                     &    77.60                                \\
% \icat{} + \knn{} (ours)    & 95.13                       &  \textbf{80.70}                                  \\ \icat{}  + \mmr{}  (ours)    &    94.96                                     &  \textbf{80.70}                                 \\ 

% \icat{} + \ftd{} (ours)    & \textbf{96.14} $\dagger$                      &   \textbf{80.70}                                 \\ 
% \hline

          
% \end{tabular}

%     \caption{Results on SVAMP - SV and MultiArith - MA.$\dagger$ indicates statistical significance over Few-shot-COT at 0.1 level (90\%).}
%     \label{tab:num_reasoning}

% \end{table}




% \begin{table}[hbt!]
% \begin{tabular}{p{5.3cm}|p{1cm}|p{1.1cm}|}
% \textbf{Method}                                           & \textbf{EM (WQA)} & \textbf{EM (MQA)} \\ \hline \hline

% \fshot{} \cite{brown2020gpt3}                             & 28.41                       & 11.66            \\
% \COT{} \cite{wei2023chainofthought}                         & 34.08                       & 20.85            \\
% Self-ask \cite{self_ask}                        & 32.58                      & 23.64            \\
% \zfshot{} \cite{kojima2023large}                          & 19.25                       & 12.22            \\ \hline

% \icat{} (text-davinci)  (ours) & 25.33 & 20.28 \\ 
% \icat{} (\flanxl{}) (ours)        &                                    &      17.92                          \\ \hline\hline
% \icat{} (ours)                 & 
% 34.00             & 25.24 $\ddagger$   \\

% \icat{} + static random (ours)       &   25.08                          &    23.24         \\
% \icat{} + random (ours)       &              29.41               & 24.36            \\
% \icat{} + \knn{} &  30.69                           & 26.99            \\
% \icat{} + \mmr{} &   30.33                                  & 27.07   \\
% \icat{} + \ftd{}         &     \textbf{36.00}                        &   \textbf{27.24}$\ddagger$               \\


% \hline            

% \end{tabular}
%     \caption{Results for Multihop QA datasets 2WikiMultihopQA - WQA and MusiqueQA - MQA. $\ddagger$ indicate statistical significance at 0.01 (99\%) over Few-shot-COT.}

%     \label{tab:complex_qa}
% \end{table}



% \begin{table}[hbt!]
% \begin{tabular}{p{5cm}|p{1cm}}
% \textbf{Method }                                            & \multicolumn{1}{c}{\textbf{EM}} \\ \hline \hline
% \multicolumn{2}{l}{\textbf{Supervised baselines} }                                                                                           \\ \hline
% FinQaNET (FinBERT)                                 & 50.10                                                                   \\
% Retriever + NeRd (BERT-base)                       & 48.57                                                                   \\ \hline
% \multicolumn{2}{l}{\textbf{Few shot prompting} }                                                                                      \\ \hline
% % GPT3 (text-davinci) (zero-shot-cot)                & 37.92                                                                   \\

% \zfshot{}                  & 47.51                                                                   \\

% \fshot{} & 42.55 \\
% \COT{} & 52.22 \\
% \icat{}  (AQUA-RAT)  (ours)      &   49.61                                                               \\
% \icat{} (TabMWP) (ours) & \textbf{53.35}                                                                  \\
%                 \hline   
% \icat{}  (text-davinci)             &  40.01                                                                       \\ \hline
% \icat{} + \knn{} (TabMWP) &     52.65                                                             \\
% \icat{} + \mmr{}{} (TabMWP) &  52.14                                                                \\
% \icat{} + \ftd{} (TabMWP) (ours) &    \textbf{55.27}$\dagger$                                                              \\ \hline

                
% \end{tabular}

%     \caption{Results for FinQA. $\dagger$ indicates statistical significance over Few-shot-COT at 0.1 level or 90\%.}

%     \label{tab:finqa}
% \end{table}
